AI-assisted coding: Experiments with GPT-4

Artificial intelligence (AI) tools based on large language models have acheived human-level performance on some computer programming tasks. We report several experiments using GPT-4 to generate computer code. These experiments demonstrate that AI code generation using the current generation of tools, while powerful, requires substantial human validation to ensure accurate performance. We also demonstrate that GPT-4 refactoring of existing code can significantly improve that code along several established metrics for code quality, and we show that GPT-4 can generate tests with substantial coverage, but that many of the tests fail when applied to the associated code. These findings suggest that while AI coding tools are very powerful, they still require humans in the loop to ensure validity and accuracy of the results.

==> _extensions/mikemahoney218/arxiv/partials/_authors.tex <==
$-- You can use as many custom partials as you need. Convention is to prefix name with '_'
$-- It can be useful to use such template to split some template parts in smaller pieces, which is easier to reuse.
$-- This '_custom.tex' is used on 'title.tex' as example.
$-- See other existing format in quarto-journals/ organisation.
$-- %%%% TODO %%%%%
$-- Use it if you need to insert content at this specific place of the main Pandoc's template. Otherwise, remove it.
$-- Here we are using it to format the authors part of the template.
$-- %%%%%%%%%%%%%%%

\textbf{$it.name.literal$}$if(it.orcid)$~\orcidlink{$it.orcid$}$endif$$for(it.affiliations/first)$\\$it.department$\\$it.name$\\$if(it.city)$$it.city$$if(it.postal-code)$,\ $it.postal-code$$endif$$endif$$endfor$\\$if(it.email)$\href{mailto:$it.email$}{$it.email$}$endif$


==> _extensions/mikemahoney218/arxiv/partials/before-body.tex <==
$-- Implements the frontmatter, title page, and abstract.
$--
$-- %%%% TODO %%%%%
$-- Customize is needed, otherwise remove this partials to use Quarto default one
$-- %%%%%%%%%%%%%%%%
$if(has-frontmatter)$
\frontmatter
$endif$
$if(title)$
$if(beamer)$
\frame{\titlepage}
$else$
\maketitle
$endif$
$if(abstract)$
\begin{abstract}
$abstract$
\end{abstract}
$endif$
$endif$
$if(keywords)$
{\bfseries \emph Keywords}
\def\sep{\textbullet\ }
$for(keywords/allbutlast)$$keywords$ \sep $endfor$
$for(keywords/last)$$keywords$$endfor$

$endif$


==> _extensions/mikemahoney218/arxiv/partials/title.tex <==
$-- Provides configuration of document metadata for writing the title block.
$-- Note that in addition to these templates and partials, Quarto will also make normalized authors and affiliations data available to the template,
$-- making is easy to write custom title blocks against a standard schema.
$--
$-- %%%% TODO %%%%%
$-- Customize is needed, like below for printing the authors. Otherwise remove this partials to use Quarto default one.
$-- %%%%%%%%%%%%%%%%
$if(linenumbers)$
\usepackage{lineno}
\linenumbers
$endif$
$if(doublespacing)$
\usepackage{setspace}
\doublespacing
$endif$
$if(date)$
\renewcommand{\today}{$date$}
$endif$
\newcommand{\runninghead}{ }
$if(runninghead)$
\renewcommand{\runninghead}{$runninghead$ }
$endif$
$if(title)$
\title{$title$$if(thanks)$\thanks{$thanks$}$endif$}
$endif$
$if(subtitle)$
\usepackage{etoolbox}
\makeatletter
\providecommand{\subtitle}[1]{% add subtitle to \maketitle
  \apptocmd{\@title}{\par {\large #1 \par}}{}{}
}
\makeatother
\subtitle{$subtitle$}
$endif$
\author{${ by-author:_authors.tex()[\\\\\\] }}
\date{$date$}

